Learning to Explain: Answering Why-Questions via Rephrasing

Providing plausible responses to why questions is a challenging but critical goal for language based human-machine interaction. Explanations are challenging in that they require many different forms of abstract knowledge and reasoning. Previous work has either relied on human-curated structured knowledge bases or detailed domain representation to generate satisfactory explanations. They are also often limited to ranking pre-existing explanation choices. In our work, we contribute to the under-explored area of generating natural language explanations for general phenomena. We automatically collect large datasets of explanation-phenomenon pairs which allow us to train sequence-to-sequence models to generate natural language explanations. We compare different training strategies and evaluate their performance using both automatic scores and human ratings. We demonstrate that our strategy is sufficient to generate highly plausible explanations for general open-domain phenomena compared to other models trained on different datasets.

==> related.tex <==
\section{Background}


% AI is basically filling in a form, rather than fully generating natural explanations: 
% Data-to-Text System.
% https://dl.gi.de/bitstream/handle/20.500.12116/16354/B1-67.pdf?sequence=1&isAllowed=y
% https://www.cambridge.org/core/services/aop-cambridge-core/content/view/2ED2083C4A62195041F527F101BB0734/S1471068413000598a.pdf/generating_explanations_for_biomedical_queries.pdf

% \subsection{Language Modeling}

% \subsection{Commonsense Reasoning Cloze Test}
% COPA
% Winograd
% getting both correct does not require generation. COPA can rely on structured models that take in causal nouns (causal net). Winograd can rely on memorizing (LM) sequence and encounter the ones that looks similar (simple method for common sense paper constructed a dataset that specifically target this). 
% common sense as "memorization" in LM
% This means we really need to sample common sense LM or use their model to rank our choices??? That sounds like a good idea :) use simple method for LM as a score ranker for our generated explanations!!!
